Theory of shock electrodialysis I: Water dissociation and electrosmotic vortices

Shock electrodialysis (shock ED), an emerging electrokinetic process for water purification, leverages the new physics of deionization shock waves in porous media. In previous work, a simple leaky membrane model with surface conduction can explain the propagation of deionization shocks in a shock ED system, but it cannot quantitatively predict the deionization and conductance (which determines the energy consumption), and it cannot explain the selective removal of ions in experiments. This two-part series of work establishes a more comprehensive model for shock ED, which applies to multicomponent electrolytes and any electrical double layer thickness, captures the phenomena of electroosmosis, diffusioosmosis, and water dissociation, and incorporates more realistic boundary conditions. In this paper, we will present the model details and show that hydronium transport and electroosmotic vortices (at the inlet and outlet) play important roles in determining the deionization and conductance in shock ED. We also find that the results are quantitatively consistent with experimental data in the literature. Finally, the model is used to investigate design strategies for scale up and optimization.

==> archived.tex <==
\begin{equation}
    \pd{(\tilde{h}\hat{c}_k)}{\tilde{t}} + \tilde{\nabla} \cdot (\tilde{h}\hat{\mathbf{J}}_k) = 0
\end{equation}
\begin{equation}
    \hat{\mathbf{J}}_{k} = \left[ \hat{\mathbf{u}}^{eff}_k  - \tilde{D}_k  \tilde{\nabla}\left(\ln (\hat{c}_k/\delta_k) + z_k  \tilde{\psi}^v \right) \right] \hat{c}_k
\end{equation}
where
\begin{equation}
    \hat{\mathbf{u}}^{eff}_k = \beta^{P}_k \hat{\mathbf{u}}^{P} +  \beta_k^{EO} \hat{\mathbf{u}}^{EO} + \sum_{l=1}^N \beta^{DO}_{kl} \hat{\mathbf{u}}^{DO}_l 
\end{equation}
The depth-averaged continuity equation should be
\begin{equation}
    \nabla \cdot \left[\tilde{h}\left(\hat{\mathbf{u}}^{P} +\hat{\mathbf{u}}^{EO} +\sum_k \hat{\mathbf{u}}^{DO}_k  \right) \right]=0
\end{equation}
where
\begin{equation}
    \hat{\mathbf{u}}^P = - \tilde{k}^P \tilde{\nabla} \tilde{p}^v
\end{equation}
\begin{equation}
    \hat{\mathbf{u}}^{EO} = - \tilde{k}^{EO} \tilde{\nabla} \tilde{\psi}^v
\end{equation}
\begin{equation}
    \hat{\mathbf{u}}^{DO}_k = - \tilde{k}^{DO}_k \tilde{\nabla} \ln \tilde{c}_k^v
\end{equation}


\subsection{Boundary conditions}{\label{sec:B.C.}}

In this part we will give the boundary conditions for the feed panel shown in Fig.\ref{fig:model}, with thin channel assumption applied. The boundary conditions at $z= 0$ and $z=h$ have been given by Eq.(\ref{eq:bc_z}) and will not be repeated here. 


At the inlet, we assume
\begin{subequations}
\begin{equation}
    u = \frac{Q}{Hh},
\end{equation}
\begin{equation}
    c_k^v = c_k^{in},
\end{equation}
\begin{equation}
    \pd{\psi^v}{x} = 0.
\end{equation}
\end{subequations}
Since we have three panels, we will specify $u^{in} = u^M$, $c_k^{in}=c_k^M$ for the main panel, $u^{in} = u^{C}$, $c_k^{in}=c_k^C$ for the cathode stream, and $u^{in} = u^A$, $c_k^{in}=c_k^A$ for the anode stream. 
At the outlet, we assume fully-developed boundary
\begin{subequations}
\begin{equation}
     p^v = p_a,
\end{equation}
\begin{equation}
    \pd{c_k^v}{x} =0,
\end{equation}
\begin{equation}
    \pd{\psi^v}{x} = 0,
\end{equation}
\end{subequations}
where $p_a$ is the atmosphere pressure. Note that $\pd{\psi}{x}=0$ at inlet and outlet is only reasonable if we assume $\sigma=0$ for the microchannels at both ends. Otherwise, non-electroneturality will lead to streaming potential gradient and we need to replace $\pd{\psi}{x}=0$ by $I_x = \int i_x dy = 0$ at the inlet and outlet, which is more complex to apply.

On all the non-penetrating walls shown in Figure xx (solid black lines, e.g. the splitter), apply
\begin{subequations}
\begin{equation}
    \mathbf{u}  \cdot \mathbf{n} = 0,
\end{equation}
\begin{equation}
    \mathbf{J}_k \cdot \mathbf{n} = 0.
\end{equation}
\end{subequations}
where $\mathbf{n}$ is the normal vector of the walls pointing to the outside of the channel. Note that on these walls we don't apply non-slip since the viscous drag on these walls to the fluid is much smaller than that on the planer walls of the nano/microchannels under the thin channel assumption. 

Finally, we need to give the upper and lower boundary conditions of the charged channel. If only two species exist (one anion, one cation), the previous work usually just assumes $J_{y, -} = 0$ (ideal cation exchange membrane) and $\psi = \pm V/2$ at the anode and cathode side. However, the ideal membrane assumption leads to almost perfect ion removal, which cannot be used to predict the magnitude of outlet concentration. Furthermore, these two boundaries are not enough for multi-component system. A possible solution is to assign artificial transference numbers
to all the ions, but it turns out this may contradict the SED performance (see xx). In this paper, we will directly simulate the transport in the membranes and electrode channels. Assume plug flow and no surface charge in electrode channels, and assume no flow in membranes (which will be justified in Sec.\ref{sec:DA}). Since the membrane is a porous material, we can use a modified homogenized model with some effective diffusivity \cite{Dydek2013NonlinearModel}. With the membrane and electrode streams modeled, we can specify the boundary conditions at the electrodes:
\begin{subequations}
\begin{equation}
    \mathbf{u} \cdot \mathbf{n} = 0,
\end{equation}
\begin{equation}
    \mathbf{J}_k \cdot \mathbf{n} = 0,  \ \ \{k = 1,2,\cdots, N_s\},
\end{equation}
\begin{equation}
    \psi^v = \pm V/2.
\end{equation}
\end{subequations}
Here we assume fast reaction on electrodes so the reaction rate is limited by ionic flux of water ions. Note that $V$ may differ from the true voltage between electrodes due to the surface over potential.
